Learning from Mixtures of Private and Public Populations

We initiate the study of a new model of supervised learning under privacy constraints. Imagine a medical study where a dataset is sampled from a population of both healthy and unhealthy individuals. Suppose healthy individuals have no privacy concerns (in such case, we call their data "public") while the unhealthy individuals desire stringent privacy protection for their data. In this example, the population (data distribution) is a mixture of private (unhealthy) and public (healthy) sub-populations that could be very different. Inspired by the above example, we consider a model in which the population $\mathcal{D}$ is a mixture of two sub-populations: a private sub-population $\mathcal{D}_{\sf priv}$ of private and sensitive data, and a public sub-population $\mathcal{D}_{\sf pub}$ of data with no privacy concerns. Each example drawn from $\mathcal{D}$ is assumed to contain a privacy-status bit that indicates whether the example is private or public. The goal is to design a learning algorithm that satisfies differential privacy only with respect to the private examples. Prior works in this context assumed a homogeneous population where private and public data arise from the same distribution, and in particular designed solutions which exploit this assumption. We demonstrate how to circumvent this assumption by considering, as a case study, the problem of learning linear classifiers in $\mathbb{R}^d$. We show that in the case where the privacy status is correlated with the target label (as in the above example), linear classifiers in $\mathbb{R}^d$ can be learned, in the agnostic as well as the realizable setting, with sample complexity which is comparable to that of the classical (non-private) PAC-learning. It is known that this task is impossible if all the data is considered private.

==> agnostic.tex <==
\subsection{Agnostic case}\label{subsec:agn}

For the agnostic setting we consider the same family of halfspaces $\wtc_{\Spub}$ as in the realizable case. Let $h_{S}^\erm$ denote the ERM halfspace w.r.t. $S$. In this setting, the sub-family $\cV$ of $\wtc_{\Spub}$ differs from the one considered in the realizable case. The subfamily $\cV$ contains halfspaces that represent the facets of the convex polytope defining the convex hull of those data points that are consistent with the ERM halfspace $h_{S}^\erm$.
Let $\olh$ denote the complement of the ERM halfspace $h_{S}^\erm$. Then, we have the following fact:

\begin{fact}\label{fact:ermempty}
	Let $\olh$ denote the complement of the ERM halfspace $h_{S}^\erm$. For $v \leq 2d \cdot \npub^d$, let $h_1, \ldots, h_v$ be the halfspaces in $\cV$, such that the intersection of these halfpsaces contains all the data points consistent with $h_{S}^\erm$. Then $ \left(\bigcap\limits_{i=1}^{v} h_i\right) \cap \olh= \emptyset$.
\end{fact}


% \begin{lem}
%  Let $\cX \subset \re^d$. Let $\cD$ be an arbitrary distribution over $\cX\times \cY \times \cP$, and let $S \sim \cD^{n}$ be the input dataset. Let $\Spub$ denote the public partition of $S$ and let $n_\pub = |\Spub|$. Let $h_{S}^\erm$ be the ERM hypothesis w.r.t. $S$. Let $\cV = \{h_1,\ldots,h_v\}$, where $v = O\left(\left(\frac{\npub}{d+1}\right)^{d+1}\right)$, such that $\Spub \subseteq \left(\bigcap\limits_{i=1}^{v} h_i\right)$. Then $ \left(\bigcap\limits_{i=1}^{v} h_i\right) \cap h_{S}^\erm= \emptyset$.
% \end{lem}

\begin{lem}
 Let $\cD$ be an arbitrary distribution over $\cX\times \cY \times \cP$, and $S \sim \cD^{n}$ be the input dataset. Let $\cV$ be the set of halfspaces in $\re^d$ as defined above. Let $h_{S}^\erm$ denote the ERM halfspace w.r.t. $S$. Then, there exists a sub-collection $\cT'$ of $\cV$ comprised of at most $d$ halfspaces denoted by $h'_1,h'_2,\ldots,h'_d$, such that $\left(\bigcap\limits_{i=1}^{d} h'_i\right)$ is consistent with $h_{S}^\erm$.
\end{lem}
\begin{proof}
Let $\olh$ denote the complement of the ERM halfspace $h_{S}^\erm$.  Let $h_1, \ldots, h_v$ be the halfspaces in $\cV$. By Fact \ref{fact:ermempty} we have, $\left(\bigcap\limits_{i=1}^{v} h_i\right) \cap \olh= \emptyset$.
Consider the collection of halfspaces in $\cV$ and $\olh$. Using Lemma \ref{lem:helly} we know that  there exists a collection $\cT$ of at most $d+1$ halfspaces whose intersection is empty.
Since the intersection of the halfspaces in $\cT$ is empty, we get that $\olh \in \cT$. 
Now consider the sub-collection $\cT' = \cT \setminus \{\olh\}$. Let the remaining $d$ halfspaces in $\cT'$ be $h'_1,h'_2,\ldots,h'_d$. Note that, $\left(\bigcap\limits_{i=1}^{d} h'_i\right)$ is a superset of the region given by intersection of the halfspaces in $\cV$. This implies that $\left(\bigcap\limits_{i=1}^{d} h'_i\right) \cap \olh = \emptyset$. Hence, $\left(\bigcap\limits_{i=1}^{d} h'_i\right)$ is consistent with $h_{S}^\erm$.
\end{proof}

\begin{thm}\label{thm:AlgAgn}
	
	Let $\cC \subseteq \{0,1\}^\cX$ be a concept class with $\vc(\cC)=d+1$. For any $\epsilon,\delta,\alpha,\beta \in (0,1)$, $\cA_\rel$ (Algorithm~\ref{alg:real}) is an $(\epsilon,\delta,\alpha,\beta)$-PAP learning algorithm for $\cC$, with input sample size $$n = O\left(\left(d^2 \log(\frac{2d^3}{\eps\alpha}) + 2\log(\frac{1}{\beta})\right)\max\left(\frac{1}{\alpha^2},\frac{1}{~\eps~\alpha}\right)\right).$$ 
\end{thm}




\anote{General case for learning halfspaces when privacy status is not fully co-related to target label. Suppose we remove some data points from the input dataset (e.g. the private data points labeled as 1). Construct a private classifier for this new distribution (tampered distribution) using similar construction. Then using transfer learning co-relate the public data points labeled as 1 to the the private data points labeled as 1. Illustrate using disease example and figure} 
